Planck pre-launch status: Design and description of the Low Frequency Instrument

In this paper we present the Low Frequency Instrument (LFI), designed and developed as part of the Planck space mission, the ESA program dedicated to precision imaging of the cosmic microwave background (CMB). Planck-LFI will observe the full sky in intensity and polarisation in three frequency bands centred at 30, 44 and 70 GHz, while higher frequencies (100-850 GHz) will be covered by the HFI instrument. The LFI is an array of microwave radiometers based on state-of-the-art Indium Phosphide cryogenic HEMT amplifiers implemented in a differential system using blackbody loads as reference signals. The front-end is cooled to 20K for optimal sensitivity and the reference loads are cooled to 4K to minimise low frequency noise. We provide an overview of the LFI, discuss the leading scientific requirements and describe the design solutions adopted for the various hardware subsystems. The main drivers of the radiometric, optical and thermal design are discussed, including the stringent requirements on sensitivity, stability, and rejection of systematic effects. Further details on the key instrument units and the results of ground calibration are provided in a set of companion papers.

==> 06_conclusions.tex <==
In this paper we have discussed the linearity properties of the Planck-LFI receivers. The voltage output has been measured during the calibration campaign of the individual receivers and of the integrated instrument using a signal input ranging from $\sim$8~K to $\sim$30~K.

The receiver response is linear for the 70~GHz receivers while the 30 and 44~GHz radiometers show non linear, compressed response over all the input signal range, which is well described by the relationship in Eq.~(\ref{eq:vout_full}). The source of signal compression has been identified in the back-end amplifiers and detector diodes and characterised by dedicated tests on two 44~GHz back-end modules.

The calculation of several performance parameters from data acquired during ground tests must take into account signal compression in order to provide a correct estimate. In particular the calculation of noise temperature, photometric calibration, white noise sensitivity and noise effective bandwidth can be completely off the correct estimates if nonlinearity is not properly taken into account.

Although compression impacts significantly the calculation of receiver performance parameters from ground test data, it is essentially negligible during nominal operations, where the input signal dynamic range is small enough ($\lesssim\pm 50$~mK) to keep the response in the linear regime. 

The last characterisation of the LFI receivers linearity will be performed during the in flight calibration exploiting the cooldown of the HFI 4~K cooler which will provide an input signal over a range from $\sim 20$~K to $\sim 4$~K.



==> 334_diode_averaging.tex <==
\bf(REVIEW THIS SECTION? - POLARISATION DIFFERENCING?)

Each radiometer produces two stable streams of sky-load differences. Further suppression of residual fluctuations can be obtained by combining the data from the two paired detectors. Performing a noise-weighted average of the two diode outputs, after calibration, helps removing systematic effects such as those due to small asymmetries in the two states of the phase switches. If $T_{w-1}$ and $T_{w-2}$ are the temperatures of input target $w$ (either sky or load) measured when the phase switch is in state 1 and
2 respectively, then we have from the two diodes A and B:
\begin{eqnarray}
    && \Delta T_B =(T_\text{sky-1}-r_B T_\text{load-2})\nonumber\\
    && \Delta T_A =(T_\text{sky-2}-r_A T_\text{load-1}).
    \label{eq:delta_ta_tb}
\end{eqnarray}

If an effect $\delta T_1$, $\delta T_2$ is introduced by a switch state such that $T_{w-1}=T_w+\delta T_1$ and $T_{w-2} = T_w + \delta T_2$, then by taking the average of the two diodes differences we have:

\begin{eqnarray}
    \frac{\Delta T_B + \Delta T_A}{2} &=& \frac{1}{2}\left[T_\text{sky} + \delta T_1 - r_B (T_\text{load} + \delta T_2)\right]+\nonumber\\
    &+&\frac{1}{2}\left[T_\text{sky} + \delta T_2 - r_A (T_\text{load} + \delta T_1)\right]+\\
    &=&(T_\text{sky}-r\, T_\text{load})\nonumber
    \label{eq:effect_double_difference}
\end{eqnarray}
% 
where here we assumed for simplicity  $r_A = r_B = r$.



==> 800_systematics_budget.tex <==
Limits on systematic effects impacting the effective angular resolution (beam ellipticity, alignment, pointing errors) were used as input to the design of the Planck telescope and focal plane, as well as to set pointing requirements at system level. From the goal limit $<$3~$\mu$K cumulative systematic error per pixel (Sect.~\ref{sec:systematics}) we defined a breakdown of contributions from various kinds of effects (Table~\ref{tab:systematics_budget}) More detailed allocations were worked out for each
contribution. This provided a useful guideline for the design, development and testing of the various LFI subsystems. For each type of
systematic error we specify limits for three cases: a high frequency component, spin-synchronous fluctuations and periodic (non-spin-synchronous) fluctuations. High frequency contributions ($\gg$0.016~Hz) can be considered as random fluctuations and added in quadrature to the radiometers' white noise. As a goal, the overall noise increase due to random effects other than radiometer white noise should be less than 10\%. Spin synchronous (0.016~Hz) components are not damped by scanning redundancy, and impose the most stringent limits to systematic effects. Periodic fluctuations on time scales other than the satellite spin are damped with an efficiency that depends on the characteristic time scale of the effect (see \citet{mennella02} for quantitative analysis).

\begin{table}[h!]
    \caption{Top level budget of LFI systematic errors. The allocated limits are residuals after consolidated software removal techniques are applied to the data}
    \label{tab:systematics_budget}
    \begin{center}
        \begin{tabular}{p{3cm} c c c}
            \hline
            \hline
            Source & Random & Spin synch & Periodic\\
                  & Fraction of $\delta T_{\rm 1-sec}$   &$\mu$K&$\mu$K\\
            \hline
            External Straylight &N/A    &1  &N/A\\
            Internal Straylight &0.045  &1  &0.9\\
            4K reference load fluctuations &0.026  &1  &0.6  \\
            LFI thermal fluctuations    &0.031  &0.8    &1.1\\
            Front end 1/f   &0.217  &N/A    &N/A \\
            Back end 1/f    &0.453  &N/A    &N/A \\
            DC electronics  &0.04   &N/A    &N/A \\
            Quantisation    &0.01   &N/A    &N/A \\
            Total   &0.507  &1.9    &1.5 \\
            Noise increase  &0.121  &   &   \\
            \hline
        \end{tabular}
    \end{center}
\end{table}



==> refs.tex <==


Jarosik et al WMAP receiver (not referenced)

Lamarre, J.M., et al 2009, A&A, This volume (need info)

Leahy et al 2009, A&A, This volume (need info)

Maffei et al 2009, A&A, This volume (need info)

Meinhold. P., et al 2009, A&A, This issue (not referenced)

Morgante, G.L., et al 2009, A&A, This issue (not referenced)

Smoot, G.F., et al COBE-DMR instrument (not referenced)

Tauber, J. et al 2009a, Pre-launch mission paper, A&A, This issue (need info)

Tauber, J. et al 2009b, Pre-launch optics paper, A&A, This issue (need info)


